Lie algebroids are curved Lie algebras

We show that there is an equivalence of $\infty$-categories between Lie algebroids and certain kinds of curved Lie algebras. For this we develop a method to study the $\infty$-category of curved Lie algebras using the homotopy theory of algebras over a complete operad.

==> macro.tex <==
%Added packages
\usepackage{todonotes}
\usepackage{mathtools}

% COMMENTS/CHANGES

\newcommand{\joost}[1]{\todo[color=green!40]{#1}}
\newcommand{\comment}[1]{\textcolor{orange}{#1}}
\newcommand{\ricardo}[1]{\todo{#1}}
\newcommand{\damien}[1]{\todo[color=blue!40]{#1}}

% MATHEMATICS

\newcommand{\K}{\mathbb{K}}

% operads
\renewcommand{\P}{\mathcal{P}}
\newcommand{\Q}{\mathscr{Q}}
\newcommand{\C}{\mathcal{C}}
\renewcommand{\O}{\mathcal{O}}
\newcommand{\com}{\mathrm{Com}}
\newcommand{\ass}{\mathrm{Ass}}
\newcommand{\lie}{\mathrm{Lie}}
\newcommand{\cocom}{\mathrm{coCom}}
\newcommand{\coass}{\mathrm{coAss}}
\newcommand{\colie}{\mathrm{coLie}}
\newcommand{\ucocom}{\mathrm{coCom}}
\newcommand{\cLie}{\mathrm{cLie}}
\newcommand{\clcLie}{\cat{cLie}_B^{\clubsuit}}%classical curved lie. Need to find a good notation
\newcommand{\End}{\mathrm{End}}
\newcommand{\coEnd}{\mathrm{coEnd}}
\newcommand{\Opns}{\mathcal{O}_{ns}}%Find better notation
\newcommand{\Opsym}{\mathcal{O}_{sym}}%Find better notation




% categories

\newcommand{\AOp}{Op^{A-aug}}
\newcommand{\ACOp}{Coop^{A-bil}}

\newcommand{\Palg}{\mathscr{P}\text{-}\mathsf{alg}}
\newcommand{\Picoalg}{\mathscr{P}^\antishriek\text{-}\mathsf{coalg}}


\renewcommand{\Bar}{\mathrm{B}}
\newcommand{\Cobar}{\Omega}

% others

\newcommand{\sym}{\mathrm{Sym}}
\newcommand{\Def}{\mathrm{Def}}
\newcommand{\MC}{\mathbf{MC}}
\newcommand{\Defsu}{\mathrm{Def}^{\mathrm{su}}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\Gr}{\operatorname{Gr}}
\DeclareMathOperator*{\id}{id}
\DeclareMathOperator{\Hom}{Hom}
\newcommand{\lieop}[1]{\mathfrak{Lie}(#1)}
\newcommand{\lieopbar}[1]{\overline{\mathfrak{Lie}}(#1)}

\newcommand{\antishriek}{\text{\raisebox{\depth}{\textexclamdown}}}
